On Some Logics Intermediate Between S4.2 and S4.3 Defined by the Notion of Independence

Hamkins and Loewe described modal logic S4.2 through the notion of sets of independent buttons - statements that are possibly necessary - and switches - necessarily contingent statements. In this article we investigate logics intermediate between S4.2 and S4.3 that are defined through a different notion of independence. We provide an axiomatic description of such logics, state some basic facts and prove various completeness and decidability results.

==> eptcsdata.tex <==
\providecommand{\firstpage}{14}
\providecommand{\publicationstatus}{A. Indrzejczak, T. Jarmu\.zek, M. Klonowski, \& M. Zawidzki (Eds.):\\ Twelfth International Conference on\\ Non-Classical Logics. Theory and Applications (NCL'26)\\
EPTCS 455, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.455.2}{10.4204/EPTCS.455.2}}
\pdfoutput=1

